Alpine Permafrost Modeling: On the influence of topography driven lateral fluxes

Alpine permafrost environments are highly vulnerable and sensitive to changes in regional and global climate trends. Thawing and degradation of permafrost has numerous adverse environmental, economic, and societal impacts. Mathematical modeling and numerical simulations provide powerful tools for predicting the degree of degradation and evolution of subsurface permafrost as a result of global warming. A particularly significant characteristic of alpine environments is the high variability in their topography and geomorphology which drives large lateral thermal and fluid fluxes. Additionally, harsh winds, extreme weather conditions, and various degrees of saturation have to be considered. The combination of large lateral fluxes and unsaturated ground makes alpine systems markedly different from Arctic permafrost environments and general geotechnical ground freezing applications, and therefore, alpine permafrost demands its own specialized modeling approaches. In this research work, we present a multi-physics permafrost model tailored to alpine regions. In particular, we resolve the ice-water phase transitions, unsaturated conditions, and capillary actions, and account for the impact of the evolving pore volume on fluid-matrix interactions. Moreover, the approach is multi-dimensional, and therefore, inherently resolves fluxes along topographic gradients. Through numerical cases studies based on the elevation profiles of the two prominent peaks of the Zugspitze (DE) and the Matterhorn (CH), we show the strong influence of topography driven thermal and fluid fluxes on active layer dynamics and the distribution of permafrost.

==> figures/benchmarks_schematic.tex <==
\begin{figure}
\centering

% TH2 
\begin{subfigure}[b]{0.75\textwidth}
\centering
\begin{tikzpicture}
\begin{scope}
\clip (0,0) rectangle (12,4);

\draw[fill=blue] (0,0) rectangle (12,4); 
\draw[fill=blue!20, color=blue!20] (3.3333, 1.3333) rectangle (4.6666,2.6666); 
\draw[] (0,0) rectangle (12,4); 

\node[] at (4,2) {-5\,$^\circ$C}; 
\node[] at (6,2) {5\,$^\circ$C}; 

\end{scope}
\end{tikzpicture}
\caption{TH2: Frozen Inclusion}
\label{fig:TH2_schematic}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.23\textwidth}
\centering
\begin{tikzpicture}
\begin{scope}
\clip (0,0) rectangle (4,4); 

\draw[fill=red!80] (0,0) rectangle (4,4);
\draw[fill=blue!20, color=blue!20] (2,-0.4) circle (2.0396);
\draw[fill=blue!20, color=blue!20] (2,4.4) circle (2.0396);

\draw[fill=black] (2,2.72) circle (0.05) node[right] {$x_2$}; 
\draw[fill=black] (2,2) circle (0.05) node[right] {$x_1$}; 
\draw[] (0,0) rectangle (4,4);

\node[] at (1,1) {-5\,$^\circ$C}; 
\node[] at (1,2) {5\,$^\circ$C}; 

\end{scope}
\end{tikzpicture}
\caption{Talik Opening/Closure}
\label{fig:TH3_schematic}
\end{subfigure}

\caption{Schematic of the benchmark test cases. The graphics \ref{fig:TH2_schematic} and \ref{fig:TH3_schematic} visualize the initial conditions of the benchmark test cases TH2 and TH3. The positions $x_1$ and $x_2$ relate to the temperature measurements of the  performance measures TH3:PM4.1 and TH3:PM4.2.} 
\label{fig:benchmark_schematic}
\end{figure}
\todo{SG: In Fig.2, for consistency with Fig.1, keep the color of the water saturated domain in 'blue' (instead of red). }




==> tex_files/supplementary_material.tex <==
%\section*{Supplementary Material}
%Nothing yet 
